Towards composition of conformant systems

Motivated by the Model-Based Design process for Cyber-Physical Systems, we consider issues in conformance testing of systems. Conformance is a quantitative notion of similarity between the output trajectories of systems, which considers both temporal and spatial aspects of the outputs. Previous work developed algorithms for computing the conformance degree between two systems, and demonstrated how formal verification results for one system can be re-used for a system that is conformant to it. In this paper, we study the relation between conformance and a generalized approximate simulation relation for the class of Open Metric Transition Systems (OMTS). This allows us to prove a small-gain theorem for OMTS, which gives sufficient conditions under which the feedback interconnection of systems respects the conformance relation, thus allowing the building of more complex systems from conformant components.

==> fromSimulation2closeness.tex <==
\subsection{From simulation to closeness}
\label{sec:fromSimulation2closeness}

In this section we show that bisimutaion implies closeness \yhl{for autonomous systems}. 
It should be emphasized that bisimulation is a relation between \emph{states}: it connects the start and end states of a transition in the MTS.
Closeness, on the other hand, is a relation between \emph{trajectories}: it connects entire trajectories starting from related initial states.
In this section we show that a bisimulation relation between states of a system is sufficient to relate their entire trajectories via closeness, under mild regularity conditions of the hybrid systems.

\begin{theorem}
\label{thm:sim implies closeness}
Take two \yhl{autonomous} hyrid systems $\Sys_1$ and $\Sys_2$ both of which satisfy Assumption \ref{ass:HBC},
and where $\Sys_2$ is derived from $\Sys_1$ with relation $D$.
Consider their OMTS embeddings $T_1$ and $T_2$ as per the procedure of Section \ref{sec:embeddingHSasOMTS}.
If $R$ is a $(\tau,\varepsilon)$-STAB relation of $T_1$ by $T_2$,
and $D \subset R$,
then $\Sys_2$ conforms to $\Sys_1$ with precision 
\yhl{
$(T,J,(2\tau,\varepsilon+\varepsilon'))$ for any $T,J \geq 0$,
where $\varepsilon' = 2\tau(\sup_{x \in C} \sup_{\zeta \in F(x)}\|\zeta\|)$.
}
\end{theorem}

%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
\ifthenelse{\boolean{REPORT}}
{\input{simu2closenessProof}}
{The proof is in the technical report~\cite{AbbasF14_HSCCTechRpt}.}
%=====================================================================================
Two remarks are in order concerning the conservatism of the conformance precision $\teps$ derived from $\teps$-simulation according to the above reasoning.

C1) First, the fact that transitions in the MTS only model forward movement of time means that the simulation relation only certifies an $\varepsilon$ obtained by forward search, whereas when computing the smallest $\varepsilon$ (for a given $\tau$) in $\teps$-closeness, one can search backward and forward in time (in a $2\tau$ window) for the closest point on the other trajectory. 
In future research we will explore the use of `backward' transitions to get tighter guarantees.
\todo[inline]{couldn't we have allowed backward labels, or does this ruin the stitching process?}
\\
C2)
\yhl{
Let $R$ be any $(\tau,\varepsilon_R)$-STAB relation between $\Sys_1$ and $\Sys_2$.
Then because $D \subset R$, $\sup_{(q_1,q_2) \in D}d_\Pi(\out{q_1^0},\out{q_2^0})\leq  \sup_{(q_1,q_2) \in R}d_\Pi(\out{q_1^0},\out{q_2^0}) \leq \varepsilon_R$.
Thus the pairs of initial states related by $D$ imply a lower bound on any precision $\varepsilon_R$ obtained by bisimulation considerations, 
even though these pairs may not be matched by closeness.
\\
C3) The inflated $\varepsilon$ can be excessively large because of the $\varepsilon'$ term, so while we have a theoretical guarantee that the systems are conformant, there is room for improvement in the numerical guarantees.
} 
%Second, the need for $D \subset R$ implies that the smallest $\varepsilon$ for which a $\teps$-simulation exists (for any $\tau$) is $\varepsilon_R \geq \sup_{D} d_\Pi(\out{q_1^0},\out{q_2^0})$.
%On the other hand, for $\teps$-closeness, we are satisfied with an $\varepsilon$ satisfying that for all $q_1^0$, $\exists q_2^0$ s.t. $q_1^0D q_2^0$ and there exists a transition $q_2^0 \trans{\slabel_2} q_2$ for which $d_{\tlabelSet}((0,0),\slabel_{2,\chi}) \leq \tau$ and $d_\Pi(\out{q_1^0},\out{q_2}) \leq \varepsilon$.
%The latter is clearly no larger than $\varepsilon_R$.

==> preliminaries.tex <==
\section{Preliminaries}
\label{sec:preliminaries}
\paragraph{Notation} We write $\Re^* = \Re \setminus \{0\}, \Re_+ =[0,\infty)$, and $\overline{\Re_+} = \Re_+ \cup \{\infty\}$.
Given $x,y \in \Re$, $x\vee y = \max\{x,y\}$ and $x \wedge y = \min\{x,y\}$.
We adopt the convention that the infimum of the empty set equals $+\infty$, and its supremum equals $-\infty$.
Given $n \in \Ne, [n] = \{1,\ldots,n\}$.
Given $x \in \Re^n$, $|x|$ is its Euclidian norm.
For a set $S$, co$S$ is its convex hull.
A \emph{set-valued} map $F: A \rightrightarrows B$ maps elements of $A$ to subsets of $B$.
%A set-valued map $F:\Re^n \rightrightarrows \Re^n$ is \emph{outer semicontinuous} if for all converging sequences $(x_i) \rightarrow x \in \Re^n$, and all sequences $(y_i) \in F(x_i)$ converging to a point $y$, it holds that $y \in F(x)$.
%It is \emph{locally bounded} if for any compact set $K \subset \Re^n$, there exists $K' \subset \Re^n$ s.t. $F(K) \defeq \cup_{x \in K} F(x) \subset K'$.
\yhl{A set-valued map $F:\Re^n \rightrightarrows \Re^n$ is \emph{bounded} if there exists a compact set $K' \subset \Re^n$ s.t.  for all compact $K \subset \Re^n$, 
$F(K) \defeq \cup_{x \in K} F(x) \subset K'$.
Its domain is the set $\{x \in \Re^n \sut F(x) \neq \emptyset\}$.}
Given a function $f:A \rightarrow B$ and $C \subset A$, $f|_C$ is the restriction of $f$ to $C$.
Given two sets $A$ and $B$ and a distance function on $A \cup B$, the Haussdorff distance between $A$ and $B$ induced by $d$ is the largest $d$-distance between any two points from each set: $d_H(A,B) = \stackrel{\rightarrow}{d_H}(A,B) \vee \stackrel{\rightarrow}{d_H}(B,A), \stackrel{\rightarrow}{d_H}(A,B) \defeq \sup_{a\in A}\inf_{b \in B} d(a,b)$.
\yhl{
A relation $R \subset A \times B$ is \emph{surjective} if for any $b\in B$, $\exists a\in A$ s.t. $(a,b)\in R$, 
and is \emph{left-total} if for any $a \in A$, $\exists b \in B$ s.t. $(a,b) \in R$.
Given $(a,b) \in A \times B$, its projections $\proj{(a,b)}{A} = a$, and $\proj{(a,b)}{B} = b$.
Given two vectors $x=(x_1,\ldots,x_n)^T$ and $y=(y_1,\ldots,y_n)^T$ of $\Re^n$, their inner product is denoted $<x,y> = \sum_i x_i y_i$.
}

\input{conformanceViaTJtec}
\input{hybridSys}




